Formalizing Event-Driven Behavior of Serverless Applications

We present new operational semantics for serverless computing that model the event-driven relationships between serverless functions, as well as their interaction with platforms services such as databases and object stores. These semantics precisely encapsulate how control transfers between functions, both directly and through reads and writes to platform services. We use these semantics to define the notion of the service call graph for serverless applications that captures program flows through functions and services. Finally, we construct service call graphs for twelve serverless JavaScript applications, using a prototype of our call graph construction algorithm, and we evaluate their accuracy.

==> simple-state-machine.tex <==
events:
  - http:
    path: signup
    method: POST
definition: 
  StartAt: RecordDB
  States:
    RecordDB:
      Type: Task
      Resource: arn:aws:lambda:us-east-1:XXXX:function:RecordDB
      Next: RecordAC
      ResultPath: $.results.RecordDB
    RecordAC:
      Type: Task
      Resource: arn:aws:lambda:us-east-1:XXXX:function:RecordAC
      End: true
      ResultPath: $.results.RecordAC
